Towards Generalized Models for Task-oriented Dialogue Modeling on Spoken Conversations

Building robust and general dialogue models for spoken conversations is challenging due to the gap in distributions of spoken and written data. This paper presents our approach to build generalized models for the Knowledge-grounded Task-oriented Dialogue Modeling on Spoken Conversations Challenge of DSTC-10. In order to mitigate the discrepancies between spoken and written text, we mainly employ extensive data augmentation strategies on written data, including artificial error injection and round-trip text-speech transformation. To train robust models for spoken conversations, we improve pre-trained language models, and apply ensemble algorithms for each sub-task. Typically, for the detection task, we fine-tune \roberta and ELECTRA, and run an error-fixing ensemble algorithm. For the selection task, we adopt a two-stage framework that consists of entity tracking and knowledge ranking, and propose a multi-task learning method to learn multi-level semantic information by domain classification and entity selection. For the generation task, we adopt a cross-validation data process to improve pre-trained generative language models, followed by a consensus decoding algorithm, which can add arbitrary features like relative \rouge metric, and tune associated feature weights toward \bleu directly. Our approach ranks third on the objective evaluation and second on the final official human evaluation.

==> overview.tex <==

% use pre-trained models
In order to build generalized models, 
we mainly employ the current state-of-the-art pre-trained language models for each task, 
followed by ensemble algorithms. 
Typically, we use \roberta~\cite{roberta}, \roberta Wide and Deep~\cite{roberta_wd},
and some variations of \roberta classification models,  
as well as generative LMs such as UniLM~\cite{unilm}, GPT2~\cite{gpt2} and DialoGPT~\cite{dialogpt}.

% an overview of our methods
Table~\ref{tab:overview} gives a brief overview of all models for all tasks. 
We divide the selection task into two sub-tasks: \textbf{Entity Tracking} and \textbf{Knowledge Ranking}.
Entity tracking aims to find a list of entities that are mentioned in a dialogue. 
With these entities, we collect all the knowledge associated with them, and 
knowledge ranking ranks those knowledge and returns top-$n$ knowledge.  
In addition to pre-trained language models, we also apply data augmentation on detection and selection tasks, 
and develop different ensemble algorithms for different tasks.

